Peculiar Motions of Galaxy Clusters in the Regions of Superclusters of galaxies

We present results of the study of peculiar motions of 57 clusters and groups of galaxies in the regions of the Corona Borealis (CrB), Bootes (Boo), Z5029/A1424, A1190, A1750/A1809 superclusters of galaxies and 20 galaxy clusters located beyond massive structures ($0.05<z<0.10$). Using the SDSS (Data Release 8) data, a sample of early-type galaxies was compiled in the systems under study, their fundamental planes were built, and relative distances and peculiar velocities were determined. Within the galaxy superclusters, significant peculiar motions along the line of sight are observed with rms deviations of $652\pm50$~km s$^{-1}$---in CrB, $757\pm70$~km s$^{-1}$---in Boo. For the most massive A2065 cluster in the CrB supercluster, no peculiar velocity was found. Peculiar motions of other galaxy clusters can be caused by their gravitational interaction both with A\,2065 and with the A2142 supercluster. It has been found that there are two superclusters projected onto each other in the region of the Bootes supercluster with a radial velocity difference of about 4000~km s$^{-1}$. In the Z5029/A1424 supercluster near the rich Z5029 cluster, the most considerable peculiar motions with a rms deviation of $1366\pm170$~km s$^{-1}$ are observed. The rms deviation of peculiar velocities of 20 clusters that do not belong to large-scale structures is equal to $0\pm20$~km s$^{-1}$. The whole sample of the clusters under study has the mean peculiar velocity equal to $83\pm130$~km s$^{-1}$ relative to the cosmic microwave background.

==> sao_cmd.tex <==
\def\saoname{Special Astrophysical Observatory of the Russian AS,
              Nizhnij Arkhyz 369167, Russia}
\def\saonamer{Специальная астрофизическая обсерватория, Нижний Архыз, 369167,
Россия}

%******* SPECIAL SIGNS AND CHARACTERS FOR MATH MODE *******
%
\def\squareforqed{\hbox{\rlap{$\sqcap$}$\sqcup$}}

\def\sq{\ifmmode\squareforqed\else{\unskip\nobreak\hfil
\penalty50\hskip1em\null\nobreak\hfil\squareforqed
\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}

\def\sun{\hbox{$\odot$}}

\def\la{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\sim\cr}}}}}

\def\ga{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\sim\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\sim\cr}}}}}

\def\degr{\hbox{$^\circ$}}

\def\arcmin{\hbox{$^\prime$}}

\def\arcsec{\hbox{$^{\prime\prime}$}}

\def\utw{\smash{\rlap{\lower5pt\hbox{$\sim$}}}}

\def\udtw{\smash{\rlap{\lower6pt\hbox{$\approx$}}}}

\def\fd{\hbox{$.\!\!^{\rm d}$}}

\def\fh{\hbox{$.\!\!^{\rm h}$}}

\def\fm{\hbox{$.\!\!^{\rm m}$}}

\def\fs{\hbox{$.\!\!^{\rm s}$}}

\def\fdg{\hbox{$.\!\!^\circ$}}

\def\farcm{\hbox{$.\mkern-4mu^\prime$}}

\def\farcs{\hbox{$.\!\!^{\prime\prime}$}}

\def\fp{\hbox{$.\!\!^{\scriptscriptstyle\rm p}$}}

\def\cor{\mathrel{\mathchoice {\hbox{$\widehat=$}}{\hbox{$\widehat=$}}
{\hbox{$\scriptstyle\hat=$}}
{\hbox{$\scriptscriptstyle\hat=$}}}}

\def\sol{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr\sim\cr<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr\sim\cr
<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr\sim\cr
<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
\sim\cr<\cr}}}}}

\def\sog{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr\sim\cr>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr\sim\cr
>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
\sim\cr>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
\sim\cr>\cr}}}}}

\def\lse{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\simeq\cr}}}}}

\def\gse{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\simeq\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\simeq\cr}}}}}

\def\grole{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\noalign{\vskip-1.5pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\noalign{\vskip-1.5pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\noalign{\vskip-1pt}<\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\noalign{\vskip-0.5pt}<\cr}}}}}

\def\leogr{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\noalign{\vskip-1.5pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\noalign{\vskip-1.5pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\noalign{\vskip-1pt}>\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\noalign{\vskip-0.5pt}>\cr}}}}}

\def\loa{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
<\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr\approx\cr}}}}}

\def\goa{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr
>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr
>\cr\approx\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr\approx\cr}}}}}

\def\diameter{{\ifmmode\mathchoice
{\ooalign{\hfil\hbox{$\displaystyle/$}\hfil\crcr
{\hbox{$\displaystyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\textstyle/$}\hfil\crcr
{\hbox{$\textstyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\scriptstyle/$}\hfil\crcr
{\hbox{$\scriptstyle\mathchar"20D$}}}}
{\ooalign{\hfil\hbox{$\scriptscriptstyle/$}\hfil\crcr
{\hbox{$\scriptscriptstyle\mathchar"20D$}}}}
\else{\ooalign{\hfil/\hfil\crcr\mathhexbox20D}}%
\fi}}

\def\getsto{\mathrel{\mathchoice {\vcenter{\offinterlineskip
\halign{\hfil
$\displaystyle##$\hfil\cr\gets\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr\gets
\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr\gets
\cr\to\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
\gets\cr\to\cr}}}}}

\def\lid{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr<\cr\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr<\cr
\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr<\cr
\noalign{\vskip1pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
<\cr
\noalign{\vskip0.9pt}=\cr}}}}}

\def\gid{\mathrel{\mathchoice {\vcenter{\offinterlineskip\halign{\hfil
$\displaystyle##$\hfil\cr>\cr\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\textstyle##$\hfil\cr>\cr
\noalign{\vskip1.2pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptstyle##$\hfil\cr>\cr
\noalign{\vskip1pt}=\cr}}}
{\vcenter{\offinterlineskip\halign{\hfil$\scriptscriptstyle##$\hfil\cr
>\cr
\noalign{\vskip0.9pt}=\cr}}}}}

%********** ABBREVIATIONS OF THE OFT-REFERENCED JOURNALS ***********

% *** Astrophysical Bulletin % англ. версия журнала САО с 2007 г.
\newcommand{\ab}{Astrophysical Bulletin}
% *** Астрофизический бюллетень % русск. версия журнала САО с 2007 г.
\newcommand{\abr}{Астрофизический бюллетень}
% *** Astronomy and Astrophysics
\newcommand{\aaa}{Astronom. and Astrophys.}
% *** Astronomy and Astrophys. Supplement Series
\newcommand{\aas}{Astronom. and Astrophys. Suppl. Ser.}
% *** Astronomy and Astrophysics Review
\newcommand{\aar}{Astronom. Astrophys. Rev.}
% *** Astronomical Journal
\newcommand{\aj}{Astronom. J.}
% *** Astrophysical Journal
%\newcommand{\apj}{Astrophys. J.}
% *** Astrophysical Journal Supplement Series
\newcommand{\apjs}{Astrophys. J. Suppl.}
% *** Astrophysics and Space Science
\newcommand{\apss}{Astrophys. and Space Sci.}
% *** Annual Review of Astronomy and Astrophys.
\newcommand{\araa}{Annu. Rev. Astronom. Astrophys.}
% *** Astronomicekij Zhurnal
\newcommand{\azh}{Astronom. Zh.}
% *** Bulletin of the American Astron. Society
\newcommand{\baas}{Bull. Amer. Astronom. Soc.}
% *** Bulletin of the Special Astrophysical Observatory % англ. версия до 2007 г.
\newcommand{\bsao}{Bull. Spec. Astrophys. Obs.}
% *** Бюллетень Спец. астрофизич. обсерватории % русск. версия до 2007 г.
\newcommand{\bsaor}{Бюлл. Спец. астрофиз. обсерв.}
% *** Inform. Bul. Var. Stars
\newcommand{\ibvs}{Inform. Bul. Var. Stars}
% *** Journal of Astronomy and Astrophysics
\newcommand{\jaa}{J. Astronom. Astrophys.}
% *** Monthly Notices of the Roy. Astron. Society
\newcommand{\mnras}{Monthly Notices Roy. Astronom. Soc.}
% *** Publ. Astronom. Soc. Japan
\newcommand{\pasj}{Publ. Astronom. Soc. Japan}
% *** Publ. of the Astron. Society of the Pacific
\newcommand{\pasp}{Publ. Astronom. Soc. Pacific}
% *** Pis'ma v Astronomicekij Zhurnal
\newcommand{\pazh}{Pis'ma Astronom. Zh.}
% *** Soviet Astronomy
\newcommand{\sovast}{Sov. Astronom.}
% *** Scientific American
\newcommand{\sca}{Scientific American}
% *** Sky and Telescope
\newcommand{\skytel}{Sky Telesc.}
% *** Space Science Reviews
\newcommand{\spsrev}{Space Sci.~Rev.}

